On Context-Dependent Clustering of Bandits

We investigate a novel cluster-of-bandit algorithm CAB for collaborative recommendation tasks that implements the underlying feedback sharing mechanism by estimating the neighborhood of users in a context-dependent manner. CAB makes sharp departures from the state of the art by incorporating collaborative effects into inference as well as learning processes in a manner that seamlessly interleaving explore-exploit tradeoffs and collaborative steps. We prove regret bounds under various assumptions on the data, which exhibit a crisp dependence on the expected number of clusters over the users, a natural measure of the statistical difficulty of the learning task. Experiments on production and real-world datasets show that CAB offers significantly increased prediction performance against a representative pool of state-of-the-art methods.

==> proofs.tex <==

\section{Proofs}\label{sa:proofs}
%
The following lemma is the starting point of our regret analysis. 
%Assume for simplicity that $||\bu_i|| = 1$ for all $i$, and that $||\bx_{t,k}|| = 1$ for all $t$ and $k = 1, \ldots, c_t$. Also, 
In what follows, $\{\cdot\}$ denotes the indicator function of the predicate at argument.
%
\begin{lemma}\label{l:instregret}
Suppose that for all $i \in \scU$, and all $\bx \in \R^d$
%, and all $t = 1, 2, \ldots$ 
it holds that
\[
|\bw_{i,t}^\top\bx - \bu_i^\top\bx| \leq \CB_{i,t}(\bx)\,.
\]
Then the regret $r_t$ the algorithm in Figure \ref{alg:tcab} incurs at time $t$ can be deterministically upper bounded as
%
\begin{align*}
r_t 
\leq 
(3\alpha(T)+2)&\Bigl( \{\hN_{i_t,t}(\bx_t^*) \neq N_{i_t}(\bx_t^*) \}\\ 
&\ \ \qquad + \{\hN_{i_t,t}({\bar \bx_t}) \neq N_{i_t}({\bar \bx_t})\} \Bigl)\\ 
&+ 2\,\CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t})~.
%\Bigl(\CB_{N_{i_t}(\bx_t^*),t-1}(\bx_t^*) + ||\bw_{N_{i_t}(\bx_t^*),t-1} - \bw_{\hN_{i_t,t}(\bx_t^*),t-1}||\Bigl)\cdot \{\hN_{i_t,t}(\bx_t^*) \neq N_{i_t}(\bx_t^*) \}\\
%&\ + \Bigl( \CB_{\hN_{i_t,t}({\bar \bx_t}),t-1}({\bar \bx_t}) + ||\bw_{\hN_{i_t,t}({\bar \bx_t}),t-1} - \bw_{N_{i_t}({\bar \bx_t}),t-1}||\Bigl)\cdot \{\hN_{i_t,t}({\bar \bx_t}) \neq N_{i_t}({\bar \bx_t})\}\,.
\end{align*}
%
\end{lemma}
%
{\em Proof.} Let $\bx_t^* = \argmax_{k = 1, \ldots, c_t} \bu_{i_t}^\top\bx_{t,k}$, so that
\[
r_t = \bu_{i_t}^\top\bx_t^* - \bu_{i_t}^\top{\bar \bx_t}\,.
\]
Then, setting for brevity
%
\begin{eqnarray*} 
N^* &=& N_{i_t}(\bx_t^*),\\
\hN^* &=& \hN_{i_t,t}(\bx_t^*),\\ 
N^- &=& N_{i_t}({\bar \bx_t}),\\
\hN^- &=& \hN_{i_t,t}({\bar \bx_t}),
\end{eqnarray*}
%
we can write
%
\begin{eqnarray*}
r_t 
&=& \bu_{i_t}^\top\bx_t^* - \bu_{i_t}^\top{\bar \bx_t}\\
&=& \frac{1}{|N^*|}\sum_{j \in N^*}\bu_j^\top\bx_t^* - \bu_{i_t}^\top{\bar \bx_t}\\
&&{\mbox{(since $\bu_j^\top\bx_t^* = \bu_{i_t}^\top\bx_t^*$ for all $j \in N^*$)}}\\
%
&=& \frac{1}{|N^*|}\sum_{j \in N^*}\bu_j^\top\bx_t^* - \bw_{N^*,t-1}^\top\bx_t^*\\ 
&&\ + \bw_{N^*,t-1}^\top\bx_t^* - \bw_{\hN^*,t-1}^\top\bx_t^*\\ 
&&\ + \bw_{\hN^*,t-1}^\top\bx_t^* + \CB_{\hN^*,t-1}(\bx_t^*)\\ 
&&\ - \CB_{\hN^*,t-1}(\bx_t^*) - \bu_{i_t}^\top{\bar \bx_t}\,.
\end{eqnarray*}
%
Using $|\bw_{j,t-1}^\top\bx_t^* - \bu_j^\top\bx_t^*| \leq \CB_{j,t-1}(\bx_t^*)$ for all $j \in N^*$, 
Cauchy-Shwartz inequality, and the definition of ${\bar \bx_t}$, the above can in turn be upper bounded by
%
\begin{align*}
&\CB_{N^*,t-1}(\bx_t^*)\\
&\quad +  ||\bw_{N^*,t-1} - \bw_{\hN^*,t-1}||\cdot \{\hN^* \neq N^* \}\\
&\quad + \bw_{\hN^-,t-1}^\top{\bar \bx_t} + \CB_{\hN^-,t-1}({\bar \bx_t})\\
&\quad - \CB_{\hN^*,t-1}(\bx_t^*) - \bu_{i_t}^\top{\bar \bx_t}\\
%
&= \Bigl(\CB_{N^*,t-1}(\bx_t^*) - \CB_{\hN^*,t-1}(\bx_t^*)\Bigl)\cdot \{\hN^* \neq N^* \} \\ 
&\quad + ||\bw_{N^*,t-1} - \bw_{\hN^*,t-1}||\cdot \{\hN^* \neq N^* \}\\ 
&\quad + \Bigl(\bw_{\hN^-,t-1}^\top{\bar \bx_t} - \bw_{N^-,t-1}^\top{\bar \bx_t}\Bigl)\cdot \{\hN^- \neq N^-\}\\
&\quad + \bw_{N^-,t-1}^\top{\bar \bx_t} + \CB_{\hN^-,t-1}({\bar \bx_t}) - \bu_{i_t}^\top{\bar \bx_t}.
\end{align*}
%
Using again Cauchy-Shwartz inequality, and $\bu_j^\top{\bar \bx_t}  = \bu_{i_t}^\top{\bar \bx_t}$ for all $j \in N^-$, the above can in turn be upper bounded by
%
\begin{align*}
\Bigl(&\CB_{N^*,t-1}(\bx_t^*) - \CB_{\hN^*,t-1}(\bx_t^*)\\ 
&\quad + ||\bw_{N^*,t-1} - \bw_{\hN^*,t-1}||\Bigl)\cdot \{\hN^* \neq N^* \}\\
&\quad + ||\bw_{\hN^-,t-1} - \bw_{N^-,t-1}||\cdot \{\hN^- \neq N^-\}\\
&\quad +  \bw_{N^-,t-1}^\top{\bar \bx_t} - \frac{1}{|N^-|}\sum_{j \in N^-} \bu_j^\top{\bar \bx_t} + \CB_{\hN^-,t-1}({\bar \bx_t})\\
%
&\leq \Bigl(\CB_{N^*,t-1}(\bx_t^*)\\ 
&\qquad + ||\bw_{N^*,t-1} - \bw_{\hN^*,t-1}||\Bigl)\cdot \{\hN^* \neq N^* \}\\
&\quad + ||\bw_{\hN^-,t-1} - \bw_{N^-,t-1}||\cdot \{\hN^- \neq N^-\} \\
&\quad + \CB_{N^-,t-1}({\bar \bx_t}) + \CB_{\hN^-,t-1}({\bar \bx_t})\\
&{\mbox{(using $|\bw_{j,t-1}^\top{\bar \bx_t} - \bu_j^\top{\bar \bx_t}| \leq \CB_{j,t-1}({\bar \bx_t})$ for all $j \in N^-$)}}\\
%
&= \Bigl(\CB_{N^*,t-1}(\bx_t^*)\\ 
&\qquad + ||\bw_{N^*,t-1} - \bw_{\hN^*,t-1}||\Bigl)\cdot \{\hN^* \neq N^* \}\\ 
&\quad + ||\bw_{\hN^-,t-1} - \bw_{N^-,t-1}||\cdot \{\hN^- \neq N^-\} \\
&\quad +  2\CB_{N^-,t-1}({\bar \bx_t})\\
&\quad + \Bigl(\CB_{\hN^-,t-1}({\bar \bx_t}) - \CB_{N^-,t-1}({\bar \bx_t})\Bigl)\cdot \{\hN^- \neq N^-\}\\
%
&\leq \Bigl(\CB_{N^*,t-1}(\bx_t^*)\\ 
&\qquad + ||\bw_{N^*,t-1} - \bw_{\hN^*,t-1}||\Bigl)\cdot \{\hN^* \neq N^* \}\\ 
&\quad + \Bigl(\CB_{\hN^-,t-1}({\bar \bx_t})\\ 
&\qquad\qquad + ||\bw_{\hN^-,t-1} - \bw_{N^-,t-1}||\Bigl)\cdot \{\hN^- \neq N^-\} \\
&\quad +  2\CB_{N^-,t-1}({\bar \bx_t})\,.
\end{align*}
%
We now handle the terms within the round braces. Since $\max_{\bx\,:\, ||\bx||=1} \bx^\top M_{i,t}^{-1} \bx \leq 1$ for all $i$ and $t$, we have that $\CB_{N^*,t-1}(\bx_t^*)$ and $\CB_{\hN^-,t-1}({\bar \bx_t})$ are both upper bounded by $\alpha(T)$. Moreover, using the shorthand $\bu_{N} = \frac{1}{|N|}\,\sum_{j \in N} \bu_j$, for $N \subseteq \scU$, we have
%
\begin{align*}
||\bw_{N^*,t-1} - \bw_{\hN^*,t-1}||
&\leq
||\bw_{N^*,t-1} - \bu_{N^*}||\\ 
&\qquad + ||\bu_{N^*} - \bu_{\hN^*}||\\ 
&\qquad + ||\bu_{\hN^*} - \bw_{\hN^*,t-1}||\\
&\leq \max_{\bx\,:\, ||\bx||\leq 1} \CB_{N^*,t-1}(\bx)\\ 
&\qquad + ||\bu_{N^*}|| + ||\bu_{\hN^*}||\\
&\qquad + \max_{\bx\,:\, ||\bx||\leq 1} \CB_{\hN^*,t-1}(\bx)\\
&\leq 2(\alpha(T)+1)~.
\end{align*}
%
Hence, we conclude that
%
\begin{align*}
r_t &\leq (3\alpha(T)+2)\left(\{\hN^* \neq N^* \} + \{\hN^- \neq N^-\} \right)\\ 
&\qquad +  2\CB_{N^-,t-1}({\bar \bx_t})~,
\end{align*}
%
as claimed. $\hfill\Box$\\
%



Under the $\gamma$-gap assumption, we also have the following lemma.
%
\begin{lemma}\label{l:1}
Let $i_t$ be the user served at time $t$ (see Figure \ref{alg:tcab}). Let
\[
|\bu_j^\top\bx - \bw_{j,t}^\top\bx| \leq \CB_{j,t}(\bx)
\]
hold for all $j \in \scU$,
%, $t = 1, 2, \ldots$, 
and $\bx \in \R^d$. Also, for fixed $\bx_t^o$, let $\CB_{j,t-1}(\bx_t^o) < \gamma/4$ holds for all $j \in \scU$. Then
\[
\hN_{i_t,t}(\bx_t^o) = N_{i_t}(\bx_t^o)~.
\]
\end{lemma}
%
{\em Proof.}
We first claim that, under the assumptions of this lemma, the following two implications hold:
%, whose proofs follow from the very same arguments as in \cite{glz14} (Lemma 4 therein):\\
\begin{enumerate}
\item[1.] Given $i,j \in \scU$, if $\bu_i^\top\bx \neq \bu_j^\top\bx$ and $\CB_{i,t}(\bx) + \CB_{j,t}(\bx) < \gamma/2$ then 
$
|\bw_{i,t}^\top\bx - \bw_{j,t}^\top\bx| > \CB_{i,t}(\bx) + \CB_{j,t}(\bx)~.
$
\item[2.] Given $i,j \in \scU$, if $|\bw_{i,t}^\top\bx - \bw_{j,t}^\top\bx| > \CB_{i,t}(\bx) + \CB_{j,t}(\bx)$ then
$
\bu_i^\top\bx \neq \bu_j^\top\bx~.
$
\end{enumerate}
%
In order to prove Item 1, notice that the $\gamma$-gap assumption entails that $\bu_i^\top\bx \neq \bu_j^\top\bx$ is equivalent to $|\bu_i^\top\bx - \bu_j^\top\bx| \geq \gamma$. Hence we can write
%
\begin{align*}
\gamma 
&\leq |\bu_{i}^\top\bx - \bu_{j}^\top\bx| \\
&\leq |\bu_{i}^\top\bx - \bw_{i,t}^\top\bx| + |\bw_{i,t}^\top\bx - \bw_{j,t}^\top\bx| + |\bw_{j,t}^\top\bx - \bu_{j}^\top\bx|\\
&\leq \CB_{i,t}(\bx) + |\bw_{i,t}^\top\bx - \bw_{j,t}^\top\bx| + \CB_{j,t}(\bx)\\
&< \gamma/2 + |\bw_{i,t}^\top\bx - \bw_{j,t}^\top\bx|~,
\end{align*}
%
implying that
\[
|\bw_{i,t}^\top\bx - \bw_{j,t}^\top\bx| > \gamma/2 > \CB_{i,t}(\bx) + \CB_{j,t}(\bx)~.
\]
As for Item 2, we can write
%
\begin{align*}
\CB_{i,t}&(\bx)  + \CB_{j,t}(\bx) 
< |\bw_{i,t}^\top\bx - \bw_{j,t}^\top\bx|\\ 
&\leq |\bw_{i,t}^\top\bx - \bu_{i}^\top\bx| + |\bu_{i}^\top\bx - \bu_{j}^\top\bx| + |\bu_{j}^\top\bx - \bw_{j,t}^\top\bx|\\
&\leq \CB_{i,t}(\bx) + |\bu_{i}^\top\bx - \bu_{j}^\top\bx| + \CB_{j,t}(\bx)~,
\end{align*}
%
implying that $|\bu_{i}^\top\bx - \bu_{j}^\top\bx| >0$. Using the above two claims, we want to show that both
%
\begin{enumerate}
\item[1a.] $N_{i_t}(\bx_t^o) \subseteq \hN_{i_t,t}(\bx_t^o)$ and 
\item[2a.] $\hN_{i_t,t}(\bx_t^o) \subseteq N_{i_t}(\bx_t^o)$
\end{enumerate}
%
hold. We choose $i = i_t$ in the above. Then, in order to prove Item 1a, we observe that if $j \in \scU$ is such that $\bu_{i_t}^\top\bx_t^o = \bu_{j}^\top\bx_t^o$ then Item 2 above implies $|\bw_{i_t,t-1}^\top\bx_t^o - \bw_{j,t-1}^\top\bx_t^o| \leq \CB_{i_t,t-1}(\bx_t^o) + \CB_{j,t-1}(\bx_t^o)$, i.e., $j \in \hN_{i_t,t}(\bx_t^o)$. On the other hand, if $j$ is such that $|\bw_{i_t,t-1}^\top\bx_t^o - \bw_{j,t-1}^\top\bx_t^o| \leq \CB_{i_t,t-1}(\bx_t^o) + \CB_{j,t-1}(\bx_t^o)$ then Item 1 above allows us to conclude that either $\bu_{i_t}^\top\bx_t^o = \bu_j^\top\bx_t^o$ or $\CB_{i_t,t-1}(\bx_t^o) + \CB_{j,t-1}(\bx_t^o) \geq \gamma/2$. Yet, because $\CB_{j,t-1}(\bx_t^o) < \gamma/4$ for all $j \in \scU$, the second conclusion is ruled out, thereby implying $j \in N_{i_t}(\bx_t^o)$.  $\hfill\Box$

\begin{remark}\label{r:1}
It is important to observe that, under the hypotheses of Lemma \ref{l:1} (when setting there $\bx_t^o = {\bar \bx_t}$), also the set of $j \in \scU $ whose profile $\bw_{j,t-1}$ gets updated at the end of round $t$ in Figure \ref{alg:tcab} coincides with $N_{i_t}({\bar \bx_t})$.
\end{remark}
%
By setting $\bx_t^o$ to either $\bx_t^*$ or ${\bar \bx_t}$, we now combine Lemma \ref{l:1} with Lemma \ref{l:instregret} to bound the number of rounds $t$ such that $\hN_{i_t,t}(\bx_t^*) \neq N_{i_t}(\bx_t^*)$ and the number of rounds $t$ such that $\hN_{i_t,t}({\bar \bx_t}) \neq N_{i_t}({\bar \bx_t})$. In turn, these will be immediately related to the hardness $\HD(\{i_t,C_t\}_{t = 1}^T,\eta)$ of the data $\{i_t,C_t\}_{t = 1}^T$ at our disposal.
%
Moreover, we will use Remark \ref{r:1} to exploit the fact that when the confidence bounds $\CB_{j,t-1}({\bar \bx_t})$ are all small enough along the selected direction ${\bar \bx_t}$, then the number of weight updates performed in round $t$ is exactly equal to the size of the true neighborhood $N_{i_t}({\bar \bx_t})$. 




{\bf Proof of Theorem \ref{t:combo}.} 
Consider the bound in Lemma \ref{l:instregret}. We can write
%
\begin{align*}
\{\hN_{i_t,t}(\bx_t^*)& \neq N_{i_t}(\bx_t^*) \}\\ 
&\leq 
\{\exists k = 1, \ldots, c_t\,:\,\hN_{i_t,t}(\bx_{t,k}) \neq N_{i_t}(\bx_{t,k}) \} \\
&\leq 
\sum_{k = 1}^{c_t} \{ \hN_{i_t,t}(\bx_{t,k}) \neq N_{i_t}(\bx_{t,k}) \} \\
&\leq 
\sum_{k = 1}^{c_t} \{\exists j \in \scU\,:\, \CB_{j,t-1}(\bx_{t,k}) \geq \gamma/4 \}\\
&{\mbox{(using Lemma \ref{l:1})}} \\
&\leq 
\sum_{k = 1}^{c_t} \sum_{j \in \scU} \{\CB_{j,t-1}(\bx_{t,k}) \geq \gamma/4 \}\,.
\end{align*}
%
Clearly, the very same upper bound applies to $\{\hN_{i_t,t}({\bar \bx_t}) \neq N_{i_t}({\bar \bx_t})\}$. Moreover,
%
\begin{align*}
\sum_{t=1}^T &\CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t}) \\
&=
\sum_{t=1}^T \{\exists j \exists k\,\,:\,\CB_{j,t-1}(\bx_{t,k}) \geq \gamma/4\}\\ 
&\qquad\qquad\qquad\qquad\times\CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t}) \\
&\quad+ \sum_{t\,:\,\CB_{j,t-1}(\bx_{t,k}) < \gamma/4\,\forall j \forall k} \CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t})\\
&\leq
\sum_{t=1}^T \sum_{k=1}^{c_t} \sum_{j \in \scU}\{\CB_{j,t-1}(\bx_{t,k}) \geq \gamma/4\}\\
&\qquad\qquad\qquad\qquad\times\max_{\bx\,:\,||\bx||\leq 1}\CB_{N_{i_t}({\bar \bx_t}),t-1}(\bx)\\
&\quad + \sum_{t\,:\,\CB_{j,t-1}(\bx_{t,k}) < \gamma/4\,\forall j \forall k} \CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t})\\
&\leq
\alpha(T)\,\sum_{t=1}^T \sum_{k=1}^{c_t} \sum_{j \in \scU}\{\CB_{j,t-1}(\bx_{t,k}) \geq \gamma/4\} \\
&\quad+ \sum_{t\,:\,\CB_{j,t-1}(\bx_{t,k}) < \gamma/4\,\forall j \forall k} \CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t})\,.
\end{align*}
%
Putting together as in Lemma \ref{l:instregret} gives 
%
\begin{align}\label{e:prebound}
\sum_{t=1}^T r_t 
&\leq 
(8\alpha(T)+4)\,\sum_{t=1}^T \sum_{k=1}^{c_t}\sum_{j \in \scU} \{\CB_{j,t-1}(\bx_{t,k}) \geq \gamma/4 \}\notag\\ 
&\quad+ 2\,\sum_{t\,:\,\CB_{j,t-1}(\bx_{t,k}) < \gamma/4\,\forall j\,\forall k } \CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t})\,. 
\end{align}
%
We first focus on the triple sum in (\ref{e:prebound}), which is easily rewritten in terms of $\HD(\{i_t,C_t\}_{t = 1}^T,\eta)$, for a suitable level $\eta$. In fact, if we denote by $\lambda_{\max}(\cdot)$ and $\lambda_{\min}(\cdot)$ the maximal and the minimal eigenvalue of the matrix at argument, we have
%
\begin{align*}
\CB_{j,t-1}(\bx_{t,k}) 
&= \alpha(t)\,\sqrt{\bx_{t,k}^\top M_{j,t-1}^{-1}\bx_{t,k}}\\
&\leq \alpha(T)\,\sqrt{\lambda_{\max}(M_{j,t-1}^{-1})}\\
&= \frac{\alpha(T)}{\sqrt{\lambda_{\min}(M_{j,t-1})}}\,,
\end{align*}
%
which is smaller than $\gamma/4$ if $\lambda_{\min}(M_{j,t-1}) > \frac{16\,\alpha^2(T)}{\gamma^2}$. Hence, recalling that $n = |\scU|$ and $c_t \leq c$ for all $t$,
%
\begin{align*}
\sum_{t=1}^T &\sum_{k=1}^{c_t}\sum_{j \in \scU} \{\CB_{j,t-1}(\bx_{t,k}) \geq \gamma/4 \} \\
&\leq
c\,n\,\HD\left(\{i_t,C_t\}_{t = 1}^T,\frac{16\,\alpha^2(T)}{\gamma^2}\right)\,.
\end{align*}
%
Next, we focus on the last sum in (\ref{e:prebound}). Let $\up(j) \subseteq \{1, \ldots, T\}$ be the set of rounds $t$ such that $\bw_{j,t}$ undergoes an update. Also, let $G = \{t = 1, \ldots, T\,:\,\CB_{j,t-1}({\bar \bx_t}) < \gamma/4\,\forall j \in \scU \}$. Notice that, for all $j \in \scU$ and $t = 1, \ldots, T$,
%
\begin{equation}\label{e:M}
M_{j,t} = I + \sum_{s \leq t\,:\,s\in \up(j)}{\bar \bx_s}{\bar \bx_s}^\top\,.
\end{equation}
%
We can write
%
\begin{align}
\sum_{t\,:\,\CB_{j,t-1}(\bx_{t,k}) < \gamma/4\,\forall j\,\forall k }& \CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t}) \nonumber\\
&\hspace{-0.7in}\leq
\sum_{t\in G} \CB_{N_{i_t}({\bar \bx_t}),t-1}({\bar \bx_t})  \nonumber\\
&\hspace{-0.7in}=
\sum_{t\in G} \frac{1}{|N_{i_t}({\bar \bx_t})|}\,\sum_{j\in N_{i_t}({\bar \bx_t})} \CB_{j,t-1}({\bar \bx_t})  \nonumber\\
&\hspace{-0.7in}=
\sum_{j \in \scU}\,\,\sum_{t\in G :j \in N_{i_t}({\bar \bx_t}) } \frac{\CB_{j,t-1}({\bar \bx_t})}{|N_{i_t}({\bar \bx_t})|} \nonumber\\
&\hspace{-0.7in}\leq 
\sum_{j \in \scU}\,\left(\sum_{t\in G:j \in N_{i_t}({\bar \bx_t})} \frac{1}{|N_{i_t}({\bar \bx_t})|^2} \right)^{1/2}\,\nonumber\\
&\times \left(\sum_{t\in G:j \in N_{i_t}({\bar \bx_t})} \CB^2_{j,t-1}({\bar \bx_t})\right)^{1/2} \label{e:twoparts}\\
&{\mbox{(from Cauchy-Shwartz inequality)\,.}} \nonumber
\end{align}
%
Now, observe that from Remark \ref{r:1}, $\{t\in G:j \in N_{i_t}({\bar \bx_t})\} \subseteq \up(j)$. Hence, for each $j \in \scU$, we have
%
\begin{align*}
\sum_{t\in G:j \in N_{i_t}({\bar \bx_t})}& \CB^2_{j,t-1}({\bar \bx_t})\\ 
&\leq 
\sum_{t\in \up(j)} \CB^2_{j,t-1}({\bar \bx_t})\\
&\leq
\alpha^2(T)\sum_{t \in \up(j)}{\bar \bx_t}^\top M_{j,t-1}^{-1}{\bar \bx_t}\\
&\leq
2\,\alpha^2(T)\log\frac{|M_{j,T}|}{|M_{j,0}|}\\
&{\mbox{(from, e.g., Lemma 24 in \cite{dgs12})}}\\
&\leq
2\,d\,\alpha^2(T)\log(1+ |\up(j)|)\\ 
&\leq  2\,d\,\alpha^2(T)\log(1+T)\,,
\end{align*}
%
where $|M|$ denotes the determinant of matrix $M$.
Furthermore, again from Cauchy-Shwartz inequality, we can write
%
\begin{align*}
\sum_{j \in \scU}\,\Biggl(&\sum_{t\in G:j \in N_{i_t}({\bar \bx_t})} \frac{1}{|N_{i_t}({\bar \bx_t})|^2} \Biggl)^{1/2} \\
&\leq
\left(n\,\sum_{j \in \scU}\,\sum_{t\in G:j \in N_{i_t}({\bar \bx_t})}\frac{1}{|N_{i_t}({\bar \bx_t})|^2} \right)^{1/2}\\
&=
\left(n\,\sum_{t\in G}\sum_{j \in N_{i_t}({\bar \bx_t})} \frac{1}{|N_{i_t}({\bar \bx_t})|^2} \right)^{1/2}\\
&\leq
\left(n\,\sum_{t=1}^T \frac{1}{|N_{i_t}({\bar \bx_t})|} \right)^{1/2}\,.
\end{align*}
%
Piecing together as in (\ref{e:twoparts}), and plugging back into (\ref{e:prebound}) gives the claimed result. $\hfill\Box$


%
{\em Proof sketch of Lemma \ref{l:anc1}. } 
% From (\ref{e:M}), we see that
% \[
% M_{j,t} \geq I + \sum_{s \leq t\,:\,i_s = j} {\bar \bx_s}{\bar \bx_s}^\top\,.
% \]
The proof is similar to that of Lemma 2 in \cite{glz14}, the main difference being in bounding the conditional expectation of $\min_{k \in \{1, \ldots, c_t\}} (\bz^\top\bx_{t,k})^2$ 
for any fixed unit-norm vector $\bz \in \R^d$. Whereas \cite{glz14} makes (strong) additional assumptions about the sub-Gaussian norm of the distribution of $X$ to prove their result, we show here that an unconditional bound is possible as well. We begin by noticing that using standard tail bounds for sub-Gaussian variables, we have, for any fixed round $t$, item index $k \in \{1\,\ldots, c_t\}$, and unit-norm $\bz \in \R^d$,
\[
\Pr_t\left( (\bz^\top\bx_{t,k})^2 > \lambda - a\,|\,(i_t,c_t) \right) \geq (1 - 2e^{-a^2/2\nu^2}),
\]
where $\Pr_t(\cdot)$ is the conditional probability
$\Pr\left(\cdot\,|\,\{i_s,C_s\}_{s=1}^{t-1}, y_1, \ldots, y_{t-1} \right)$. Since the context vectors are (conditionally) independent, this gives us the lower bound
%
\begin{align*}
\Pr_t&\left(\min_{k \in \{1,\ldots,c_t\}}(\bz^\top\bx_{t,k})^2 > \lambda - a\,|\,(i_t,c_t) \right)\\ 
&\geq \max\left\{0,(1 - 2e^{-a^2/2\nu^2})^c\right\}\,.
\end{align*}
%
Now, since $\min_{k \in \{1,\ldots,c_t\}}(\bz^\top\bx_{t,k})^2$ is a positive random variable, we use the above bound on its complementary cumulative distribution function to bound its expectation. 
%Let $K$ be an upper bound on the number of items being recommended at any time step, i.e. $c_t \leq K$ for all $t$. 
If $\E_t[\cdot]$ denotes the conditional expectation $\E\left[\cdot\,|\,\{i_s,C_s\}_{s=1}^{t-1}, y_1, \ldots, y_{t-1} \right]$, we can write
%
\begin{align*}
\E_t&\left[\min_{k \in \{1\,\ldots, c_t\} }(\bz^\top\bx_{t,k})^2\,|\,(i_t,c_t) \right]\\
& = \int_{0}^{\infty} \Pr_t\left(\min_{k \in \{1,\ldots,c_t\}} (\bz^\top\bx_{t,k})^2 > \zeta \,|\,(i_t,c_t) \right)\,d\zeta\\
& \geq \int_{0}^{\lambda} \Pr_t\left(\min_{k \in \{1,\ldots,c_t\}} (\bz^\top\bx_{t,k})^2 > \zeta \,|\,(i_t,c_t) \right)\,d\zeta\\
& \geq \int_{0}^{\lambda} \max\left\{0,(1 - 2e^{-(\lambda-\zeta)^2/2\nu^2})^c\right\}\,d\zeta\\
& =: C(\lambda,\nu,c)\,. 
\end{align*}
%
The proof then continues as in Lemma 2 of \cite{glz14} by setting up a Freedman-style tail bound to get, as a consequence of the above, the following high-confidence estimate, holding with probability at least $1-\delta$, uniformly over $j \in \scU$, and $t = 1, 2, \ldots, $:
%
\begin{align}
&\min_{k_1 \in \{1,\ldots,c_1\}, \ldots, k_t \in \{1,\ldots,c_t\}} 
\lambda_{\min}\left(I + \sum_{s \leq t\,:\,i_s = j} \bx_{s,k_s} \bx_{s,k_s}^\top \right)\notag\\
&\geq 1 + B_{\lambda,\nu,c}\left(T_{j,t},\frac{\delta}{2nd}\right)~,\label{e:mineigen}
\end{align}
%
where
%
\begin{align*}
B_{\lambda,\nu,c}&(T,\delta)\\ 
&= C(\lambda,\nu,c)\,T - 8\left(\log(T/\delta) + \sqrt{T\,\log(T/\delta)} \right)\,.
\end{align*}
%
We continue by lower bounding (\ref{e:mineigen}) with high probability. Observe that, for any fixed $j$ and $t$, variable $T_{j,t}$ is binomial with parameters $t$ and $1/n$. Let us define the auxiliary function
\[
D(x) = 2n\left(x+\frac{5}{3}\log\left(\frac{Tn}{\delta}\right) \right) 
= \scO\left( n x+n\log\left(\frac{Tn}{\delta}\right) \right)~.
\]
A standard application of Bernstein inequality to (Bernoulli) i.i.d. sequences allows us to conclude that, for any fixed value $x$,
%
\begin{equation}\label{e:bern}
\Pr(\exists j \in \scU,\,\exists t > D(x)\,:\, T_{j,t} \leq x) \leq \delta~.
\end{equation}
%
Now, in order for (\ref{e:mineigen}) to be lower bounded by $\eta$ for all $j \in \scU$ with probability at least $1-\delta$, it suffices to have
\[
T_{j,t} = \Omega \left(\frac{\eta}{C^2(\lambda,\nu,c)}\,\log\left(\frac{nd}{\delta}\right)\right) := x^*~.
\] 
We set $x = x^*$ into (\ref{e:bern}) to conclude that when
\[
t \geq D(x^*) = \Omega \left(\frac{n\,\eta}{C^2(\lambda,\nu,c)}\,\log\left(\frac{Tnd}{\delta}\right)\right)
\]
then
\[
\HD\Bigl(\{i_t,C_t\}_{t = 1}^T,\eta \Bigl) = \scO\left(\frac{n\,\eta}{C^2(\lambda,\nu,c)}\,\log\left(\frac{Tnd}{\delta}\right)\right)~,
\]
as claimed $\hfill\Box$




{\em Proof sketch of Lemma \ref{l:anc2}. } 
%
Fix round $t$, let
$\E_t[\cdot]$ denote the conditional expectation $\E\left[\cdot\,|\,\{i_s,C_s\}_{s=1}^{t-1}, y_1, \ldots, y_{t-1} \right]$,
and define 
\[
Z_{t,k} = \frac{1}{|N_{i_t}(\bx_{t,k})|} - \E_t\left[\frac{1}{|N_{i_t}(\bx)|}\,|\, (i_t,c_t) \right]~,
\]
Since $Z_{t,k}$ is a centered sub-Gaussian random variable, by a standard maximal inequality (e.g., Lemma 2.3 in \cite{m07}) we have that
%
\begin{align}
\E_t\Bigl[ & \frac{1}{|N_{i_t}({\bar \bx_t})|} \,|\, (i_t,c_t) \Bigl] \notag\\
&\leq 
\E_t\left[ \max_{k = 1, \ldots, c_t} \frac{1}{|N_{i_t}(\bx_{t,k})|} \,|\, (i_t,c_t) \right]\notag\\
&\leq 
\E_t\left[ \frac{1}{|N_{i_t}(\bx)|} \,|\, (i_t,c_t) \right] + \sqrt{\frac{2\,\nu'\,\ln c}{n}}~.\label{e:expectation}
\end{align}
%
Then, defining the variables
\[
D_t = \frac{1}{|N_{i_t}({\bar \bx_t})|} -  \E_t\left[\frac{1}{|N_{i_t}({\bar \bx_t})|}\,|\, (i_t,c_t) \right]~,
\] 
for $t = 1,\ldots, T$,
we have that $D_1, \ldots, D_T$ are a martingale difference sequence to which we can apply standard concentration inequalities.
In particular, in the light of (\ref{e:expectation}), . . .








***


{\bf Proof of Corollary \ref{c:1}.} 

****


==> results.tex <==


first 20\% for parameter tuning and rest for test (figures only display on test)


\subsection{Results}
The results are summarized in Figure~\ref{fig:results}. For the online advertising data sets Tuenti, KDD Cup and Avazu datasets, we measured performance using the Click-Through Rate (CTR). For the LastFM dataset we measured the the cumulative reward. We were particularly interested in the behavior of the competing algorithms in the cold-start settings to assess their ability to exploit collaborative effects.

In all four datasets, CAB was found to offer superior or competitive performance as compared to all baselines. CAB was found to have a much more significant improvement on the Tuenti dataset, offering almost double the CTR as compared to some of the baselines, than on the KDD Cup dataset. This is expected since exploiting collaborative effects becomes more important on a dataset like Tuenti where users are exposed to a few ($\approx$ 100) ads as compared to the KDD datasets which has a much broader ad base ($\approx$ 7000). This shows that CAB effectively exploits collaborative effects when it is most crucial.

CAB was also found to offer benefits in the cold-start region (i.e., the first relative small fraction of time horizon) on all the datasets. Moreover, the variants ...
%\cabo and 
%\cabt, 
... 
continue to maintain a lead. This is most readily apparent in the LastFM dataset where ... 
%\cab 
consistently leads in terms of cumulative rewards. Notice that algorithms such as LinUCB-SINGLE/MULTIPLE, which do not incorporate collaborative effects, give extremely poor results on all datasets. This highlights the importance of incorporating collaborative effects into recommendation.



